Taming Resource Heterogeneity In Distributed ML Training With Dynamic Batching

Current techniques and systems for distributed model training mostly assume that clusters are comprised of homogeneous servers with a constant resource availability. However, cluster heterogeneity is pervasive in computing infrastructure, and is a fundamental characteristic of low-cost transient resources (such as EC2 spot instances). In this paper, we develop a dynamic batching technique for distributed data-parallel training that adjusts the mini-batch sizes on each worker based on its resource availability and throughput. Our mini-batch controller seeks to equalize iteration times on all workers, and facilitates training on clusters comprised of servers with different amounts of CPU and GPU resources. This variable mini-batch technique uses proportional control and ideas from PID controllers to find stable mini-batch sizes. Our empirical evaluation shows that dynamic batching can reduce model training times by more than 4x on heterogeneous clusters.

==> cloud-eval.tex <==
\subsection{Cloud Evaluation}

Experiments in the cloud environment based on the policy section writeup.

For initial resource allocation ~\ref{subsec:init-alloc} :

\textbf{1. How Heterogeneity is useful.}

Simultaenous preemptions vs. partial failures.
ASP will be easier to evaluate because it will scale.

Intent is to show that training can continue with partial failures.

Measure: Cost, training curve

contender 1 : Simult. preemptions on homogenous plus restart.
contender 2 : Partial preemptions on heterogenous without restart (ASP) 
This suffers from the Heterogeneity performance overhead. 
contender 3: Same Heterogeneous cluster but with uniform batching, to show benefit of variable batching

\sahil{contender_1: you mean stop ALL VMs, then relaunch ALL of them to resume training?  I have heterogeneous VMs on cloud, so you're saying that I spawn 10 homogeneous VMs and do this there?
contender_2: you mean just put 1 VM out of commission and let training continue (with SAME batch-size as before) ?}

Should already have results for contenders 2 and 3?

\sahil{No for 2. Ran heterogeneous setup but NO premptions were made. Need to run this. I have 3.}

For homogenous case: checkpointing is an option that can help. But ckpt frequency is important. Will lose some progress. Can estimate the homogenous running time (or atleast Throughput) based on ckpt frequency.

It is possible that homogenous setup outperforms omniML because of the heterogeneity penalty? Few ways to address this:

1. Use VMs of same computing power but in different avail zones.
2. Only two types of VMs, so less heterogeneity.
3. 

\textbf{2. Early readjustment policy.}

Run larger number of preemptible VMs based on the policy. 
Let some die. 
Then readjust batch sizes for the ``stable'' configuration.  

QS: Do we adjust on every preemption or nah? If we do, this makes little sense.
Otherwise what we are saying is that we also ``batch'' the readjustments and not do it for every server preemption.

QS: How long to wait. Find inflection point? Depends on the market. etc.

Start on preemptible. Lots will fail.
Two cases. 1. Replenish with a different server type.
2. Dont replenish.

In both cases, batch size readjustment required. We can do both, but what is the message going to be? Both replenishment policies can benefit from batch adjustment? 

Eager replenishment vs. inflection point based policy comparison.

Homogen cluster ok? 
ASP, since we want to tolerate the preemptions.

Say 10 VMs originally.
Within 1 hour, 4 are terminated.
Eager policy rebalances batches 4 times.
Our lazy policy waits for 1 hour and then does a single rebalance. 

\sahil{since you mentioned a homogen cluster, they start with same batch-size. so is work adjusting or conserving? meaning is B the same value as before? and after
4 are terminated, remaining 6 are adjusted to B? what do you mean by eager policy rebalances batches 4 times?? didn't find lazy policy in policy.tex. can you explain this?}


\textbf{GPU + large collection of preemptible CPUs?}

For some extra cost, can provide a good speedup.

Ignore if the local cluster GPU + CPU expts are sound and complete.

\sahil{I've uploaded GPU experiments executed on  cloud and local cluster (with only 1 GPU worker, 1 GPU and 1 CPU worker, and 4 GPU workers in google sheets. Is this gonna be enough?). No expts done on mixed GPUs and CPUs on cloud though. }

\textbf{3. Elasticity and noise scale }

Experiment: With different batch sizes (small, v. large) show that the noise based scaling can indeed improve performance.

Some workers are preempted.

BSP should be fine? 

For small B, dont decrease the batch size.
For large B, can decrease the batch size.

Cloud is not necessary. Local cluster should be ok. 

Start with original cluster of say 3 workers (homogenous is fine?).

Preempt one of them 

There are thus four cases.


\begin{enumerate}
\item Start with a small B. After preemption, keep B.
  \item Start with a small B. After preemption, reduce B.
\item Start with large B. After preemption, keep B.
\item Start with large B. After preemption, reduce B.
\end{enumerate}

Ideally, configs 1 and 4 should outperform 2 and 3 respectively?

\sahil{Out of total 3 workers, will preempt JUST 1. gonna return a given accuracy and TTA for the 4 runs? should be enough?}


\textbf{4. Deflation adjustment}

Deflate, show that we can still adjust and the throughput is maintained compared to uniform batching. Start with homogenous cluster.

Run on local CPU cluster. 
Multiple ways to deflate.
1. For the running docker container, decrease its CPU allocation.
2. Run an interference workload using lookbusy or some other load generator tool.
3. Use hard resource limits, and start another docker container

Compare:

\begin{enumerate}

\item   Uniform batching base case
\item  Dynamic batching
\item  (Maybe) variable batching based on the amount deflated. This will lead to suboptimal batch sizes, but final result may not be too different wrt dynamic batching.

\sahil{understood. will do uniform and dynamic. gonna put a pin on variable for now.}

\end{enumerate}
  
Deflate once the training curve stabilizes, so after an hour or so?



==> conclusion.tex <==
\vspace*{\subsecspace}
\vspace*{\subsecspace}
\section{Conclusion}
\vspace*{\subsecspace}

This paper presents the notion of dynamic mini-batch sizes for distributed data-parallel training, that adjusts the mini-batch sizes on workers based on resource availability.
This technique is able to alleviate the stragglers and staleness in distributed training in various static and dynamic heterogeneous environments.
Our empirical evaluation shows that dynamic mini-batching can improve performance by upto $4\times$ compared to current uniform batching approaches. 

\vspace*{\subsecspace}

==> impl.tex <==
\section{Implementation}
%\label{sec:impl}

We have implemented the dynamic batching mechanism and various policies as part of our OmniLearn system that is based on TensorFlow v 1.14. 
%
We build on top of TensorFlow's Estimator API~\cite{tf-estimator}, and implement the dynamic batching controller in about a 1000 lines of code. 

%Additionally, if we consider the code we wrote/modified for the three workloads, that should add about another 1000 lines of code. Including the scripts for dynamically spawning workers locally and on the cloud would add another 700 lines of code outside of Tensorflow.
%

%\textbf{Explain Estimator integrationin few lines. Where are major changes made}

If a change in any worker's mini-batch size is required (as per the controller output), then we  need to checkpoint, terminate, and restart the training process.
This is due to TensorFlow's execution model which builds the computational graph based on the input mini-batch size and doesn't permit changing the mini-batch size within a session. 
% This is because the input function is defined and called only once during the training and evaluation phase. It cannot be modified once the execution graph is created. 
% This design hindered our objective of dynamically adjusting the batches on a per-worker basis and hence, we use a kill-restart approach, where we checkpoint and terminate the training on all workers, and resume training with the updated batch sizes via warm-starting mechanism.
This kill-restart mechanism contributes to a small performance overhead \emph{between 0.38-1.4\%}, since the mini-batch updates are infrequent thanks to the dead-banding technique. 
%We found that the overhead of using this strategy was \emph{between 0.38-1.4\%} of the total execution time on the opposite end of the heterogeneity level spectrum.  


To measure the iteration times on each worker, we measure the execution time on the compute\_gradients operation on each worker. We did this since computing the gradients is one of the most compute intensive operations in deep learning. In order to determine the time taken to compute gradients, we run tracing at each step. The delta between the time of the last and the first op in the graph pertaining to the compute\_gradients namescope is the time we're interested in.
To carry out tracing, we specified FULL\_TRACE in the \texttt{tf.RunOptions} and \texttt{tf.RunMetadata}.
We do this on a per-step basis using a \texttt{tf.compat.v1.train.MonitoredSession} from inside the  \texttt{tf.estimator.train\_and\_evaluate} to start model training and evaluation. The batch-sizes are specified  via \texttt{tf.estimator.TrainSpec}. We also add a \emph{node\_batch\_size} option in \texttt{tf.estimator.RunConfig} for per-worker mini-batch sizes.

\begin{comment}
Since our control mechanism relies on accurate iteration times, we record the duration of the compute\_gradients TensorFlow operation, which does not include the gradient aggregation time. In case of BSP, this aggregation time is the time taken by the slowest worker since parameter server waits until all the workers complete training on that step.

This was crucial to implement dynamic batching in ASP as well as BSP. Simply logging the start and end time to execute the train\_op in the \texttt{MonitoredSession} run call worked for ASP, but not for BSP. In the Estimator framework, the train\_op time includes the time to parse the input batch, calculate the gradients, send gradients to the parameter server, update weights, and finally send back the updated weights to the workers. 

The per-step gradient computation time varies on each worker since compute\_gradients is the major compute intensive training phase. Hence, workers with more resources are able to complete a training step quickly than others. In ASP, aggregating time over the complete step (computing and applying gradients) works fine, but in BSP, the parameter server keeps an accumulator which waits for all workers (or specified explicitly in \texttt{SyncReplicasOptimizer}  with replicas\_to\_aggregate option) to send their gradient updates and only then sends the updated weigths to all the workers to move training to the next step. Hence, the total train\_op time on each worker is equal to the time taken by the slowest worker in the cluster to send its gradient update to the parameter server. For this reason, we implement tracing to measure the time taken exclusively by each worker on training the network.

We implement dynamic batching controller that constantly monitors the cluster and adjusts either with ASP or BSP synchronization mechanism whenever necessary. The adjustment is triggered whenever the current performance of any worker gets affected (in incremental or decremental fashion) due to either resource deflation, inflation, overcommitment or interference. To enable dynamic batching, a user has to specify the four parameters: window size, threshold, adjustment mode and synchronization mode. The window size specifies the number of training steps/iterations to consider before making an adjustment check. Dynamic batching can be enabled at every step as well by specifying a window size of 1. The adjustment mechanism specifies the technique to use for readjustment: either exponential smoothing or dead-banding. Batch-size bounds are implemented by default in both the mechanisms. The controller can either start training with sub-optimal batch-sizes (uniform batch-sizes on all workers) or computes the initial mini-batch allocation based on computing capacities (core counts and FLOPs) of different workers.

The threshold is the minimum value to cross to trigger a readjustment.
In case of exponential smoothing, the threshold denotes the ratio of a worker computation time to the average cluster, while in case of dead-banding, the threshold denotes the minimum delta between the old batch-size and the new adjusted batch-size. If absolute value of delta is greater than or equal to the threshold, we execute the readjustment. Last, the synchronization mode can be either ASP or BSP to trigger the appropriate strategy.

We run multiple thresholds that can be specified with exponential smoothing and dead-banding. In case of exponential smoothing, we observed that using a higher threshold value like 0.5 made the adjustments appropriate at higher HLs, but made our controller unable to detect system disparity at low HLs. On the other hand, specifying a value too low made adjustments too frequent. For example, with HL 2 with ASP and threshold of 0.1, readjustment occur once every 100 steps. When we set the threshold to 0.3, only three adjustments were made throughout the training phase before the system converged to the ideal batch-sizes given the batch-size bounds. No deflation or interference occurred during this time. A three worker cluster of workers with (4,4,8) cores CPU running Resnet-50 with dynamic batching ASP and threshold of 0.3 initiated with a suboptimal batch-size of 128 converged to a value (93,81,210). With variable batching, the batch-sizes would be (96,96,192). Hence, compared to variable batching, dynamic batching brings us even closer to the ideal batches while still maintaining the bounds. 

\end{comment}

Each worker is run inside a docker container for ease of management and configuration. To enable communication between the docker container, we created an attachable overlay network on top of docker swarm. The CPU and memory allocation for each container is specified via --cpus and --mem options respectively. In summary, the controller implements the lazy pre-emption handling policy, manages the global batch-size, and handles all dynamic resource availability.

==> impl2.tex <==
\vspace*{\subsecspace}
\vspace*{\subsecspace}
\section{Implementation}
\label{sec:impl}


We have implemented the dynamic batching mechanism and various policies as part of our OmniLearn system that is based on TensorFlow 1.14. 
%
We build on top of TensorFlow's Estimator API~\cite{tf-estimator}, and implement the dynamic batching controller in about a 1000 lines of code. 
The controller measures and collects the iteration times of all the workers, computes the new batch sizes, and when required, reconfigures the training to use the updated batch sizes. 


To measure the iteration time on each worker, the execution time of TensorFlow's \texttt{compute\_gradients} operation is recorded using the internal performance tracing framework. 
% Importantly, this measures only the gradient computation time and does not account for the blocked time in BSP,
The controller runs as part of the master process, and computes the batch sizes using the techniques from the previous section.
Due to the deadbanding (Section~\ref{subsubsec:control-stability}), small variations in batch sizes are ignored, and updates are rare. 



If a change in any worker's mini-batch size is required (as per the controller output), then we  need to checkpoint, terminate, and restart the training process.
This is due to TensorFlow's execution model which builds the computational graph based on the input mini-batch size and doesn't permit changing the mini-batch size within a session.


% This is because the input function is defined and called only once during the training and evaluation phase. It cannot be modified once the execution graph is created. 
% This design hindered our objective of dynamically adjusting the batches on a per-worker basis and hence, we use a kill-restart approach, where we checkpoint and terminate the training on all workers, and resume training with the updated batch sizes via warm-starting mechanism.
This kill-restart mechanism contributes to a small performance overhead \emph{between 0.38-1.4\%}, since the mini-batch updates are infrequent thanks to the dead-banding technique. 
%We found that the overhead of using this strategy was \emph{between 0.38-1.4\%} of the total execution time on the opposite end of the heterogeneity level spectrum.  
New mechanisms that allow dynamic batch sizes \emph{without} the above kill-restart technique can improve the responsiveness of the controller, since the lower overhead will allow us to reduce the deadband size and make finer, more frequent adjustments. 
%
Finally, the controller specifies mini-batch sizes for each worker via the \texttt{TF\_CONFIG} environment variable.
%
The controller also picks up the various control parameters such as the batch size change threshold via this environment variable. 

% We implement dynamic batching controller that constantly monitors the cluster and adjusts either with ASP or BSP synchronization mechanism whenever necessary. The adjustment is triggered whenever the current performance of any worker gets affected (in incremental or decremental fashion) due to either resource deflation, inflation, overcommitment or interference. To enable dynamic batching, a user has to specify the four parameters: window size, threshold, adjustment mode and synchronization mode. The window size specifies the number of training steps/iterations to consider before making an adjustment check. Dynamic batching can be enabled at every step as well by specifying a window size of 1. The adjustment mechanism specifies the technique to use for readjustment: either exponential smoothing or dead-banding. Batch-size bounds are implemented by default in both the mechanisms. The controller can either start training with sub-optimal batch-sizes (uniform batch-sizes on all workers) or computes the initial mini-batch allocation based on computing capacities (core counts and FLOPs) of different workers.


==> macros.tex <==
\newcommand{\sysname}{OmniML\xspace}

%\newcommand{\comment}[1]{{\color{blue}[\textsf{#1}]}}

%\newcommand{\TODO}[1]{\comment{TODO: #1}}
%\renewcommand{\paragraph}[1]{\textbf{#1}}


\RequirePackage[normalem]{ulem}
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1}
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}}
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}
%DIF SAFE PREAMBLE
\providecommand{\DIFaddbegin}{}
\providecommand{\DIFaddend}{}
\providecommand{\DIFdelbegin}{}
\providecommand{\DIFdelend}{}
%DIF FLOATSAFE PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}
\providecommand{\DIFaddbeginFL}{}
\providecommand{\DIFaddendFL}{}
\providecommand{\DIFdelbeginFL}{}
\providecommand{\DIFdelendFL}{}
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

\def\Section {\S}

\newcommand{\squishlist}{
 \begin{list}{$\bullet$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{3pt}
     \setlength{\topsep}{3pt}
     \setlength{\partopsep}{0pt}
     \setlength{\leftmargin}{1.5em}
     \setlength{\labelwidth}{1em}
     \setlength{\labelsep}{0.5em} } }
	
\newcommand{\squishlisttwo}{
 \begin{list}{$\bullet$}
  { \setlength{\itemsep}{0pt}
     \setlength{\parsep}{0pt}
    \setlength{\topsep}{0pt}
    \setlength{\partopsep}{0pt}
    \setlength{\leftmargin}{2em}
    \setlength{\labelwidth}{1.5em}
    \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
  \end{list}  }

\newcommand{\alert}[1] {\textcolor{red} {\textsc{#1}}}

\newcommand{\myfbox}[1] {\noindent \fbox{\parbox{0.5\textwidth} {#1}}}

\newcommand{\mhead}[1] {\noindent \textbf{#1}}

\newcommand*\mean[1]{\overline{#1}}

\newcommand{\eat}[1]{}

\newcommand{\compresslist}{%
  \setlength{\itemsep}{1pt}%
  \setlength{\leftmargin}{1.5em}
  \setlength{\labelwidth}{1em}
  \setlength{\parskip}{0pt}%
  \setlength{\parsep}{0pt}%
%  \setlength{\itemindent}{-10pt}%
}

\newcommand{\myfigspace}[0]{-0.3cm}
\newcommand{\bigfigspace}[0]{-0.5cm}
\newcommand{\captionspace}[0]{-0.22cm}
\newcommand{\subsecspace}[0]{-5pt}
\newcommand{\eqspace}[0]{-5pt}
\newcommand{\largesubsecspace}[0]{-0.42cm}

==> policy.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Dynamic Batching Policies For Cloud Environments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% one page or so huh


The dynamic batching technique is particularly useful in cloud and shared data center environments where there is static heterogeneity and  dynamic resource availability. 
%
Dynamic batching can be integrated with cloud resource management, and permits many cloud deployment capabilities and scenarios, which we describe in this section.  
%
We first look at how we can integrate with existing optimized provisioning techniques for transient resources, and then describe policies for handling various voluntary and involuntary resource elasticity scenarios.



\begin{comment}
technique permits many cloud deployment capabilities and scenarios.
In this section, we describe how it can be integrated with and improve cloud resource management for distributed training.
We first look at how initial resource allocation policies with dynamic batching, 
This dynamic availability, also known as elasticity, can either result from voluntary application bursting policies, or be externally induced by the resource provider.
For instance, voluntary elastic scaling can be used in the cloud by distributed training when the cost of computing resources (i.e., cloud VMs) drops. % can take advantage of
Inversely, low-cost transient resources, that are ideal for distributed training, can be unilaterally reclaimed by the resource provider.
The dynamic batching mechanism can be adapted to different resource provisioning and elasticity scenarios, which we describe in the rest of this section.
Multiple phases of the lifecycle of distributed training applications on the cloud have different forms of heterogeneity.
The typical workflow involves initial resource allocation that minimizes cost; reacting to VM preemptions or VM deflation.
We describe each of these three components next. 
\end{comment}

%\noindent \textbf{Initial Resource Allocation.}
\subsection{Initial Resource Allocation} % For Heterogeneous Training}
\label{subsec:init-alloc}

The ability to run on heterogeneous clusters comprised of servers with different resource capacities is crucial for cloud-native applications.
%
When running on low-cost preemptible cloud VMs, there is a risk of concurrent or simultaneous preemptions that stops all forward progress.
%
These concurrent preemptions can occur if the demand for the VMs greatly exceeds the supply.
%
For instance, since GPU-enabled VMs are nearly universally used by ML applications, they are in high demand.
%
Relying solely on them can result in total resource unavailability, and thus poses a high unavailability risk to the application.


It is thus necessary to \emph{diversify} the transient resources used by distributed applications, which reduces the risk of complete resource unavailability.
%
If we use VMs of different resource configurations (types), then training can still continue even if one VM type becomes unavailable. 
%
Thus most state of the art transient resource allocation techniques use this resource diversification, and optimize the selection of VMs of different types that minimizes both the cost and the risk of simultaneous preemptions.
%
In general, lowering this risk requires a higher degree of diversification and cluster heterogeneity.
%
A recent approach in transient computing is to construct multiple server \emph{portfolios} with different cost and preemption risk, which the applications then choose based on their risk tolerance.
%
Briefly, we select a portfolio $\mathbf{x}$ minimizes $\text{Cost}(x) + \alpha\cdot\text{Risk}(x)$.
%
The $\alpha$ parameter controls the relative importance of revocation risk, and higher values result in lower risk and higher heterogeneity portfolios~\cite{exosphere}. 


For distributed training, in addition to cost and preemption risk, heterogeneity also affects the performance.
%
Our dynamic batching technique is compatible with, and can be directly incorporated into portfolio based VM selection.
%
The output of portfolio selection is a list of $(\alpha, [x_1, x_2,\ldots,x_m])$, where $\alpha$ is the risk tolerance of the portfolio, and $x_i$ represents the number of servers of type $i$ to be selected.
%
Since the resource configurations of each VM type are available, we initialize the mini-batch sizes on all the workers based on the VM's core count.
%
If the portfolio contains GPU VMs, then we use half-precision floating point performance instead of core counts for the mini-batch allocation.


While dynamic batching can be used for distributed training on \emph{any} heterogeneous cluster, there is some performance overhead due to Heterogeneity even with dynamic batching.
%
We thus select portfolios with a lower heterogeneity level when possible, since the performance overhead of highly heterogeneous clusters can increase running time and cost. 
This is easily accomplished in portfolio based allocation by setting a low value of $\alpha$. 


\begin{comment}
Necessary to have heterogeneous clusters. Feasible with our mechanism.
Illustrate how to do it. Portfolio.  Alloc average batch size and distribute it. Througput prop var batching. How to handle preemptions. Cluster size changes, and you do dynamic batching. (isnt this in next subsec) 
Cluster and server diversification is essential when running on preemptible servers to avoid concurrent failures. 
Concurrent failures significantly reduce the resource availability. 
If diversification is not used, then if the supply of VMs of that type is affected, then all VMs are lost and the training cannot make any progress. 
For general transient resource allocation, a risk vs. return tradeoff exists, and servers of different resource configurations have lower correlation of simultaneous preemption.
Dynamic batching is an ideal solution for the optimized heterogeneous clusters that result from current resource allocation policies such as portfolios and others.
Without variable mini-batch sizes, heterogeneity would result in a very high performance penalty.
Past work on diversified resource allocation has assumed fungible resources and has assumed that heterogeneity does not impose any performance penalty.
Therefore for those principles to be still viable, the degradation due to heterogeneity should be minimized, which we can provide.
Thus dynamic batching is compatible with existing initial resource allocation policies.
\end{comment}

% Talk about the nursery idea here? Or later




%\noindent \textbf{Reacting to Preemptions.}
\subsection{Resource Elasticity}

% Motivation and context. Where it exists. voluntarily vs. involuntary


Long-running distributed training workloads face frequent and many forms of dynamic resource availability in modern data center and cloud environments. 
%
This resource scaling can be voluntary or involuntary, and involve either increasing or decreasing the resources, and in all cases results in dynamic resource heterogeneity. 
%
We now describe how the dynamic batching technique can be adapted to different cases of dynamic heterogeneity due to the resource elasticity.
 

%\subsubsection{Reacting to Resource Reclamation}

%Resources can be reclaimed either through outright preemptions or fractionally with deflation. 

\subsubsection{Reacting to Preemptions.}
If a subset of VMs are preempted, this can change the heterogeneity of the cluster.
Preemptions should therefore trigger a redistribution of the mini-batches among the remaining workers. 
We therefore compute the new mini-batch sizes as part of the dynamic batch adjustment, and resume the training with the new batch sizes if required. 
Note that since we use a deadband for the batch sizes, if the preemption doesnt substantially change the resource distribution among the workers, then no actual batch adjustment will be made.


%
Our policy's reaction also depends on the kind of synchronization used. 
With BSP, any worker preemption requires stopping the training on all the remaining workers and resuming from a previous checkpoint.
In contrast, with ASP, training can continue on the remaining workers.

Each readjustment of batch sizes requires stopping and restarting all the workers, which increases the training time slightly (\~1 minute).
An \emph{eager} readjustment policy recomputes the batch sizes after every preemption, which can increase the training time overhead. 
However, the tradeoff is that readjusting the batches also improves the parallel and statistical efficiency.

\begin{comment}
We thus implement a \emph{lazy readjustment policy} when reacting to preemptions.
This policy applies to ASP, since for BSP, training has to be terminated and resumed anyway, and we always recompute the batch sizes. 
For ASP, the utility of variable batching is lower than for BSP, which makes this policy more appealing.

This lazy readjustment policy is particularly well suited for bathtub preemption rates that are found in Google Preemptible VMs, that have a high rate of initial preemptions.
That is, Google Preemptible VMs are more likely to be preempted immediately after launching them.
Therefore, our lazy preemption policy waits until this early preemption phase, and then readjusts the batches.
Thus, the frequent early preemptions do not trigger an expensive and low-utility termination+restart.

We use a preemption probability model of Google's Preemptible VMs from~\cite{} to calculate how long to wait for before triggering the lazy readjustment.
Specifically, we find the inflection point of the preemption rate curve, and wait till this inflection point is reached.
Since the preemption rates and thus the inflection point of the VMs are different, we wait till the maximum of inflection points of all the VM types. 
\end{comment}


\subsubsection{Reacting to Deflation}
VM deflation is a recently proposed approach in which VM resources are fractionally reclaimed, which results in dynamic resource availability for the application. 
Since different VMs can be deflated to different levels at the same time, this also results in dynamic heterogeneity.
Our policy for reacting to deflation events is straight-forward: we trigger the dynamic batch readjustment after every deflation/reinflation event.
Ofcourse small changes in the resource allocation will be naturally ignored due to the deadbanding in our batch size controller.










% since training  and restarting from a previous checkpoint. This is also an opportunity to readjust the mini-batch sizes on all the workers and increase their batch sizes. 

% Restarting is not necessary for ASP since training can continue on the remaining workers.
% %
% Tradeoff is that readjusting batch size involves terminating and restarting the training which adds a small performance overhead.
% However not doing so leads to training with suboptimal mini-batch sizes which can increase training time.
% %

% To optimize this tradeoff, we develop a policy for ASP training for minimizing the impact due to restarting. 

% Our policy for ASP training is especially tailored to scenarios where preemptions are bunched up. 


% We also develop a special policy for non-memoryless preemptions such as found in Google Cloud Platform.
% High initial rate of failures.
% Thus our policy calls for provisioning a larger cluster than is required, and then once the VMs ``mature'', we readjust the the batch sizes once the cluster is in a ``steady state''.
% This is mainly applicable for ASP since the resumption overhead is minimal and this is thus a ``special case'' since we anticipate a large number of preemptions in a short window. For BSP need to restart anyway, so we adjust batch size on all adjustments anyway. 

% Some sort of equation can come here. CDF model, double derivative, inflextion point. Max of all. Less than one hour. Overhead with these policies assuming a constant kill-restart overhead. 

% Overhead of restart is constant.
% Penalty of inappropriate batch size.
% This looks like some kind of dynamic programming...ski rental or something like that. Not too dissimilar to the optimal checkpointing...




% Preemptions result in a decrease in the number of workers.
% The lost servers can be replenished by using servers of other types.

% This is a form of elasticity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Global Batch Size Scaling}

Large changes in cluster configuration and resource availability occur also require policies for workload scaling.
In the context of distributed training, this entails changing the global batch size (i.e., sum of mini-batches of all workers) to match the new resource availability.

Such application directed workload (i.e., global batch size) scaling imposes a few additional challenges to SGD based training because the speedup is not proportional to the batch size, especially for larger batches, due to fundamentally stochastic nature of SGD. 
That is, increasing the global batch size by a factor of $k$ does not necessarily reduce the training time by $k$, and for larger batch sizes, the reduction in training time is $<<k$.

With dynamic resource availability we face two choices for adjusting the global batch size.
The first option is ``batch size conserving''---which maintains the intial global batch size even after resource availability has changed. 
The second option is ``batch size scaling''---which adjusts the global batch size based on change in resource availability. This maintains the average mini-batch size. 
For example, the batch size scaling policy will decrease the global batch size by half when half the VMs are preempted, and the mini-batch size on the remaining workers does not change. 

Both the options (conserving and scaling) have their tradeoffs, especially in case of deflation or preemption. 
With the size conserving policy, the individual mini-batches on the workers increase and the remaining workers can get overloaded. 
Processing large batches can reduce the throughput of overloaded workers due to memory constraints.


%On the other hand, with batch size scaling, the workers not be over or under loaded, but 

Our global batch size policy does size conservation by default, since the global batch size is an important hyperparameter carefully chosen in conjunction with other parameters such as learning rate, and we do not want to perturb the training configuration.
After the mini-batch readjustment, we monitor the throughputs of the individual workers.
If the throughput drops, then we scale down the global batch size to be proportionate to the actual resource availability. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}

When the cluster faces a change in total resource availability, we face two choices for how to proceed. 
The total batch size can either be maintained or adjusted to the changed resources. 
We use a two step approach. 
We continue running with original batch size.
This can result in some workers being overloaded. 
The throughput on those workers will drop, and we then scale back and instead rescale the batch size and adjust the total batch size to the new resource availability.
We do this if we anticipate that the new batch sizes will cause some bounds to be hit.
Even if no bounds are hit, thput may still drop, and our policy helps in catching that. 

Initial global batch size $B_0$.
With proportional scaling, we'd get $(1-f)B_0$ where $f$ fraction of resources were reclaimed .
Choice is whether to stick to original global batch size or not, considering the above tradeoff of overloading workers.
We scale back the batch size if we know that reducing it will not hurt training performance.
To determine this, we use the gradient noise scale.
For the given model, we compute $B_{\text{noise}}$ and shrink if we are still smaller than the noise scale.

The noise scale is approximated by using linear interpolation and averaging the estimates. Useful since we have various batch sizes throughout the history of the training.



\textbf{Explain why this total-batch tradeoff is important.}
Lowering batch sizes lowers the throughput.
But relation between batch size and training quality is not straight forward. SGD errors accumulate with larger batch sizes.
Also larger batch sizes have higher risk of stragglers.
Thus need to be judicious. 


  
Can be fine tuned and adjusted for different heterogeneous configurations.

In this section, we discuss the interaction with cloud based execution. 

\subsection{Cloud resource allocation}

Allows transient servers to be used effectively. Can mix different types of GPUs and CPUs etc to reduce the fault-tolerance overhead.
Any heterogeneous cluster configuration can be used. 
Performance with Heterogeneity is quite bad even 

Choose according to portfolio allocation.
Get portfolio vec.
Then, 


\subsection{Cloud Elasticity}

Can integrate with GCP preemptible. That is, keep a bunch of VMs running. Then expand the cluster with stable VMs... New technique is not cost based but availability and preemption probability based...

QS: faul  tolerance overhead. Wasting time on idling servers... disrupts all workers. Better to be stable instead. 

Can anything about the dynamic batching technique help with elasticity, or be integrated with it? 


If cluster size changes, then

Work adjusting: $\sum b$ is constant. 
Work conserving: $\bar{b}$ is constant.

For cloud elasticity, we can use the batch size bounds to determine whether to scale or not. 

Important implications for the batch size vs. SGD error arguments. 

Read the sysml elasticity paper.... 

\subsection{Deflation}

Deflation signal sent to the ML framework.
Act as explicit trigger for readjustment, although not strictly required.
Because this is loss of resources, only affected workers batch size is changed.
Other workers dont increase their batch size and are not penalized.
% This can go either way realy.. 

With deflation the decision is either voluntarily reduce work, or be overcommitted. Supports black-box deflation without reconfiguring worker. 

This is more like an empirical experiment than a nuanced policy. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

Variable batching mechanism helps dampen the impact of heterogeneity and allows for more informed resource allocation.
%
Especially valid in cloud environments, where computing resources have different tradeoffs and require selection of heterogeneous clusters for smooth operation.
%
Servers of a single type may all be revoked simultaenously---especially GPU VMs that are all in high demand.
%
By diversifying, training can continue.
%
A popular way is to run on highly heterogeneous clusters. % This sounds like an introduction...
%
However as we have seen, heterogeneous clusters are bad for training.
%
Our dynamic batching mechanism can however help in alleviating heterogeneity-induced performance degradation.
%

We now present a resource allocation policy that minimizes the cost of training.
%
Based on portfolio approach that has been used in transient server context earlier [sigmetrics and hpdc].
%
However, performance agnostic and fungible resources etc.
%

Three way tradeoff: cost, performance, and revocation risk.


May need some systems contributions in this paper and this is where we can add them?

Portfolio based construction? Combining with Hyperparameter search?

\end{comment}


  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

